OnePose: One-Shot Object Pose Estimation without CAD Models

We propose a new method named OnePose for object pose estimation. Unlike existing instance-level or category-level methods, OnePose does not rely on CAD models and can handle objects in arbitrary categories without instance- or category-specific network training. OnePose draws the idea from visual localization and only requires a simple RGB video scan of the object to build a sparse SfM model of the object. Then, this model is registered to new query images with a generic feature matching network. To mitigate the slow runtime of existing visual localization methods, we propose a new graph attention network that directly matches 2D interest points in the query image with the 3D points in the SfM model, resulting in efficient and robust pose estimation. Combined with a feature-based pose tracker, OnePose is able to stably detect and track 6D poses of everyday household objects in real-time. We also collected a large-scale dataset that consists of 450 sequences of 150 objects.

==> fig/supp_ba_align.tex <==

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{fig/orig_images/supp_ba_align.pdf}
    \caption{
    \textbf{Alignment quality across sequences.} Triangulated point clouds from one sequence are projected to images from another sequence of the same object. 
    The quality of alignment can be measured by the differences between projected 3D points (in blue) and the original 2D keypoints (in red) on the images.
    }
      \vspace{-0.5 cm}
    \label{fig:ba_align}
\end{figure}



==> fig/supp_pvnet.tex <==

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{fig/orig_images/supp_pvnet_mask.pdf}
    \caption{
    \textbf{Examples of generated masks for PVNet training.} The generated masks are overlayed on the original image in blue.
    }
      \vspace{-0.5 cm}
    \label{fig:mask_example}
\end{figure}



==> tab/supp01_hloc.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{c||ccc|ccc|ccc|c} 
\hline
\multirow{2}{*}{\#Samples} & \multicolumn{3}{c|}{Large Objects}                  & \multicolumn{3}{c|}{Medium Objects}          & \multicolumn{3}{c|}{Small Objects}          & \multicolumn{1}{l}{\multirow{2}{*}{Time (\textit{ms})}}  \\ 
\cline{2-10}
                             & 1cm-1deg        & 3cm-3deg        & 5cm-5deg        & 1cm-1deg & 3cm-3deg        & 5cm-5deg        & 1cm-1deg & 3cm-3deg        & 5cm-5deg       & \multicolumn{1}{l}{}                                     \\ 
\hline
\multicolumn{11}{c}{HLoc \textit{(SIFT + NN)}}                                                                       \\ 
\hline
2    & 0.214 & 0.418 & 0.449 & 0.292 & 0.489 & 0.519 & 0.177 & 0.357 & 0.398 & 47.79 \\
5     & 0.311 & 0.559 & 0.597 & 0.346 & 0.571 & 0.610 & 0.223 & 0.429 & 0.487 & 116.27
  \\
10    & 0.359 & 0.622 & 0.668 & 0.384 & 0.608 & 0.649 & 0.228 & 0.443 & 0.507 & 218.82   \\
\hline
\multicolumn{11}{c}{HLoc \textit{(SPP + NN)}}                                                                       \\ 
\hline
2     & 0.257 & 0.486 & 0.517 & 0.350 & 0.538 & 0.561 & 0.229 & 0.455 & 0.524 & 54.61\\
5      & 0.333 & 0.618 & 0.661 & 0.425 & 0.654 & 0.693 & 0.304 & 0.576 & 0.651 & 136.98
  \\
10    & 0.388 & 0.682 & 0.730 & 0.464 & 0.707 & 0.747 & 0.325 & 0.609 & 0.705 & 231.89
 \\
\hline
\multicolumn{11}{c}{HLoc \textit{(SPP + SPG)}}                                                                       \\ 
\hline
2                            & 0.308           & 0.553           & 0.584           & 0.438    & 0.618           & 0.628           & 0.294    & 0.542           & 0.619          & 221.43                                                   \\
5                            & 0.426           & 0.789           & 0.835           & 0.541    & 0.779           & 0.815           & 0.390    & 0.711           & 0.822          & 555.56                                                   \\
10                           & 0.479           & 0.846           & 0.879           & 0.580    & 0.839           & 0.869           & 0.422    & 0.754           & 0.876          & 1094.25                                                  \\
\hline
\end{tabular}
}
\caption{\textbf{Experiment on the effects of number of images sampled (i.e., retrieved) for HLoc.} 
We evaluate our visual localization baselines based on HLoc\cite{sarlinCoarseFineRobust2019} with differnt number of images sampled.
}
\label{tab:exp_abl_visloc}
\end{table*}
